Playing Against Fair Adversaries in Stochastic Games with Total Rewards

We investigate zero-sum turn-based two-player stochastic games in which the objective of one player is to maximize the amount of rewards obtained during a play, while the other aims at minimizing it. We focus on games in which the minimizer plays in a fair way. We believe that these kinds of games enjoy interesting applications in software verification, where the maximizer plays the role of a system intending to maximize the number of "milestones" achieved, and the minimizer represents the behavior of some uncooperative but yet fair environment. Normally, to study total reward properties, games are requested to be stopping (i.e., they reach a terminal state with probability 1). We relax the property to request that the game is stopping only under a fair minimizing player. We prove that these games are determined, i.e., each state of the game has a value defined. Furthermore, we show that both players have memoryless and deterministic optimal strategies, and the game value can be computed by approximating the greatest-fixed point of a set of functional equations. We implemented our approach in a prototype tool, and evaluated it on an illustrating example and an Unmanned Aerial Vehicle case study.

==> prob_almost_sure_system.tex <==
\section{Almost-Sure Failing Systems} \label{sec:prob_almost_sure}

Probabilistic masking simulation determines whether a fault-tolerant
implementation is able to completely mask faults.  However, in
practice, this kind of masking fault-tolerance is uncommon. Usually,
fault-tolerant systems are able to mask a number of faults before
suffering a failure. Our main goal in this section is to extend the
game theory presented in the previous section to be able to measure
the amount of masking tolerance exhibited by a system before it fails.
To do this, we extend the probabilistic masking games with a
quantitative objective function.  This is done in such a way that the
expected value of this function indicates the number of ``milestones''
that the fault-tolerant implementation is expected to cross before
failing.  A milestone is any interesting event that may occur during
the execution of the system.  For instance, a milestone may be the
number of faults occurring during the execution of the system, and
therefore this measure will reflect the number of faults that are
tolerated by the system before crashing. Another milestone may be
successful acknowledgments in a transmission protocol, in this case we
measure the expected number of chunks that the protocol is able to
transfer under the occurrence of faults before finally failing.


To do this type of measuring, we need a stochastic games with a
quantitative objective function.  This objective function counts the
number of ``milestones'' observed during a play.
%
Therefore, we first extend stochastic masking game as follows.

\remarkPRD{no tiene sentido incluir la reward function ya que est\'a completamente definida por el conjunto de milestones}

\begin{definition}%
  Let
  $A =( S, \Sigma, \rightarrow, s_0 )$ and $A' =( S', \SigmaF, \rightarrow', s_0' )$
  be two PTSs.
%
  A \emph{stochastic masking game graph with milestones} $\mathcal{M}$
  is a tuple
  $\MilestoneG_{A,A'} = (V^\StochG, E^\StochG, V^\StochG_\Refuter, V^\StochG_\Verifier, V^\StochG_\Probabilistic, \InitVertex, \delta^\StochG, r^\StochG, \mathcal{M})$
  where:
  \begin{inparaenum}[(i)]
  \item%
    $(V^\StochG, E^\StochG, V^\StochG_\Refuter, V^\StochG_\Verifier, V^\StochG_\Probabilistic, \InitVertex, \delta^\StochG)$  is a stochastic masking game graph,
  \item%
    $\mathcal{M} \subseteq \SigmaF^2$ is the set of \emph{milestones}, and
  \item%
    $\reward^\StochG(v) = (\chi_{\mathcal{M}}(\pr{1}{v}), \chi_{\ErrorSt}(v))$ is the \emph{reward function}.
  \end{inparaenum}
\end{definition}
%
In the definition above, $\chi_B$ is the characteristic function over
set $B$, defined as usual:
$\chi_B(a) = {(a{\in}B)}\mathbin{?}1\mathbin{:}0$.
If $B=\{b\}$ is a singleton set, we simply write $\chi_b$.





\hrmkPRD{VOY POR AQUI}










Note that the reward function returns a pair of numbers instead of a
single number. It is direct to codify this pair into a number, but we
do not do it here for the sake of clarity. 
	
	Given a stochastic masking game graph with milestones and reward function $r^\StochG$. For any play 
$\rho = \rho_0, \rho_1,  \dots$,
we define the \emph{masking payoff function} as follows:
\[
	\FMask(\rho) = \lim_{n \rightarrow \infty} (\sum^{n}_{i=0} \pr{0}{r_i}) \pr{1}{r_n}
\] 
where 
$r_i = \reward^\StochG(\rho_i)$,  for all $i \geq 0$.

%\[
%\FMask(\rho) = \lim_{n \rightarrow \infty}  \frac{\pr{1}{v_n}}{2^{\sum^{n}_{i=0} \pr{0}{v_i}}}.
%\]
	Intuitively, the payoff function defined above characterizes the number of milestones that a fault-tolerant implementation is able to achieve until the
error state is reached. One may think of this as a game played by the fault-tolerance built-in mechanism and a (malicious) player that chooses the 
way in which faults occur. In this game, the Verifier is the maximizer (she intends to obtain as much milestones as possible) and the 
Refuter is the minimizer (she intends to prevent the Verifier from achieving milestones).



We only focus on almost-sure failing systems, that is, systems that
eventually fail with probability 1.  This is a fairly reasonable
assumption for systems expected to operate indefinitely.


	Formally, we are interested in those cases in which the expected value of $\FMask(\rho)$ is defined. As shown below, one of these cases 
is when the probability of reaching the error state is $1$. Let us formally characterize this kind of systems.
\begin{definition}  Let $A =( S, \Sigma, \rightarrow, s_0 )$ and $A' =( S', \SigmaF, \rightarrow', s_0' )$ be two PTSs. We say that $A'$ is an \emph{almost-sure failing implementation}  of $A$ iff, 
for every strategies $\strat{\Verifier} \in \Strategies{\Verifier}, \strat{\Refuter} \in \Strategies{\Refuter}$, it holds: $\Prob_{\strat{\Verifier},\strat{\Refuter}}(\mathcal{A})=1$ where $\mathcal{A} = \{ \rho= \rho_0,\rho_1,\dots \mid \exists i \geq 0: \rho_i=\ErrorSt \text{ and }  \rho \text{ is a path in } \MilestoneG^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}\}$.
\end{definition}
The following theorem states that for almost-sure failing implementations the expected value of $\FMask$ is well-defined. The proof of this theorem consists in reducing stochastic masking
games to \emph{transient games} as presented in \cite{FilarV96}. A full proof of this result can be found in \cite{CastroDPD20}.
\begin{theorem}\label{theo:determined} Given a stochastic masking game with milestones  $\MilestoneG_{A,A'} = (V^\StochG, E^\StochG, V^\StochG_\Refuter, V^\StochG_\Verifier, V^\StochG_\Probabilistic, \InitVertex, \delta^\StochG, r^\StochG, \mathcal{M})$ for some PTSs $A$ and $A'$.
	If $A'$ is an almost-sure failing implementation of $A$; then, for every pair of strategies $\strat{\Verifier}, \strat{\Refuter}$, $\mathbb{E}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]$ is defined. Furthermore:
\[\adjustlimits
	\inf_{\strat{\Refuter}} \sup_{\strat{\Verifier}} \mathbb{E}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] = \adjustlimits \sup_{\strat{\Verifier}} \inf_{\strat{\Refuter}}  \mathbb{E}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]
\]
\end{theorem}
%\begin{proof} For proving the theorem let us consider the subgame $\mathcal{H}_{A,A'}$ obtained from $\MilestoneG_{A,A'}$ by restricting the successors of Verifier's vertices to the following
%sets:
%\begin{itemize}
%	\item $\{ ((s, \sigma^2, s', \mhyphen, \mu', \mhyphen, \Verifier), (s, \#, s', \mu, \mu', w, \Probabilistic)) \mid (\exists\;\sigma \in \Sigma: s \xrightarrow{\sigma} \mu) \wedge  \wedge w \in \vertices{\couplings{\mu}{\mu'}}\} \subseteq E^\StochG$ for any $\sigma \notin \faults$,
%
% 	 \item $\{ ((s, \sigma^1, s', \mu, \mhyphen, \mhyphen, \Verifier),(s, \#, s', \mu, \mu', w, \Probabilistic)) \mid (\exists\;\sigma \in \Sigma: s' \xrightarrowprime{\sigma} \mu' ) \wedge  w \in \vertices{\couplings{\mu}{\mu'}} \} \subseteq E^\StochG$,
%	 
%	 \item $\{ ((s, F^2, s', \mhyphen, \mu', \mhyphen, \Verifier), (s, \#, s', \delta_s, \mu', w, \Probabilistic)) \wedge w \in \vertices{\couplings{\delta_s}{\mu'}} \} \subseteq E^\StochG$ for any $F \in \faults$,
%\end{itemize}
%That is, we restrict the couplings to the vertices of the polytope $\couplings{\mu}{\mu'}$. Let us note that since the set of vertices is finite, the game  $\mathcal{H}_{A,A'}$ is finite. We also remove 
%transition $(\ErrorSt, \ErrorSt)$ from the edges of $\mathcal{H}_{A,A'}$. Let us note that  $\mathcal{H}_{A,A'}$  is a
%\emph{transient stochastic game}, as defined in \cite{CompetitiveMarkovChain}, i.e., $\sum^{\infty}_{i=0} \mathbf{P}^i_{\strat{\Verifier},\strat{\Refuter}}$ is finite, where $\mathbf{P}^i_{\strat{\Verifier},\strat{\Refuter}}$ is
%the stochastic matrix corresponding to the Markov chain $\mathcal{H}^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}$. Indeed, as proven in \cite{Condon92}, for stochastic games that halt with probability $1$ we have that $(I -  \mathbf{P}^i_{\strat{\Refuter},\strat{\Verifier}})^{-1}$ exists,
%and therefore (by Lemma~2.4.2 in \cite{CompetitiveMarkovChain}) we have that $\sum^{\infty}_{i=0}  \mathbf{P}^i_{\strat{\Verifier},\strat{\Refuter}}$ is finite. Hence, by Theorem~4.2.6 in \cite{CompetitiveMarkovChain},
%$\mathcal{H}_{A,A'}$ is determined, and the value $\mathbb{E}_{\mathcal{H}_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]$ is defined for every strategies $\strat{\Verifier},\strat{\Refuter}$. 
%
%	Now, let us observe that, for any distributions $\mu:S\rightarrow [0,1]$, $\mu':S'\rightarrow [0,1]$,  $w \in \couplings{u}{u'}$ there is
%a $w' \in \vertices{\couplings{u}{u'}}$ such that $w'(s,s') \geq w(s,s')$ for all $s,s'$ (maximums and minimums of $\couplings{u}{u'}$ are attained at the vertices). That is, for any
%cylinder $\text{Cyl}(v_0,v_1,\dots,\ErrorSt)$ in $\MilestoneG^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}$ we have a cylinder $\text{Cyl}(v'_0,v'_1,\dots,\ErrorSt)$ in $\mathcal{H}_{A,A'}$ such that:
%if $v_i$ is a Refuter's node or a Verifier's node then $v_i=v'_i$, if $v_i$ is a probabilistic node then $\pr{5}{v_i}(v_0,v_1) \leq \pr{5}{v'_i}(v_0,v_1)$ for all Refuter's nodes $v_0$ 
%and $v_1$ (note that Verifier's and Refuter's nodes coincide in both $\MilestoneG^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}$ and $\mathcal{H}^{A,A'}$). Hence:
%\begin{align*}
%	\mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] = & \\
%	  = & \int_\Omega \FMask  \mathrm{d} \Prob{\strat{\Verifier}}{\strat{\Refuter}} &  \\
%	%  = & \int_{\bigcup\{\text{Cyl}(v_0, v_1, \dots \ErrorSt) \mid v_0, v_1, \dots \ErrorSt \in \Omega_{\MilestoneG^{\sigma,\pi}_{A,A'}}\}} \FMask d \Prob{\sigma}{\pi} &  \\
%	  = & \sum_{\rho{.}\ErrorSt \in (V^{\MilestoneG^{\strat{\Refuter},\strat{\Verifier}}_{A,A'}})^* } \Prob{\strat{\Verifier}}{\strat{\Refuter}}(\text{Cyl}(\rho{.}\ErrorSt))* \FMask(\rho{.}\ErrorSt) &\\
%	  \leq &\sum_{\rho{.}\ErrorSt \in (V^{\mathcal{H}^{\strat{\Refuter},\stratprime{\Verifier}}_{A,A'}})^*} \Prob{\strat{\Verifier}}{\strat{\Refuter}}(\text{Cyl}(\rho{.}\ErrorSt))* \FMask(\rho{.}\ErrorSt)& \\
% 	 = & \mathbb{E}_{\mathcal{H}_{A,A'}}^{\stratprime{\Verifier},\strat{\Refuter}}[\FMask] & 
%\end{align*}
%	Where $\stratprime{\Verifier}$ is a Verifier's strategy such that, if  $\strat{\Verifier}(v) = (s,\#,s',\mu,\mu',w)$ then $\stratprime{\Verifier}(v) = (s,\#,s',\mu,\mu',w')$ for
%$w(t,t') \leq w'(t,t')$ for every $(t,t') \in S \times S'$ (by the remarks above we known that there is such a strategy). Thus $\mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]$
%is defined. 
%
%	For the second part of the theorem. The inequality: $\inf_{\strat{\Verifier}} \sup_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] \leq \sup_{\strat{\Refuter}} \inf_{\strat{\Verifier}}  \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]$ holds. Now, we have that: 
%\[ 
%\sup_{\strat{\Verifier}} \mathbb{E}_{\mathcal{H}_{A,A'}}^{\strat{\Verifier}, \strat{\Refuter}}[\FMask] \leq \sup_{\strat{\Verifier}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask],
%\] 
%for any Refuter's strategy $\strat{\Refuter}$, since the Verifier's strategies $\strat{\Verifier}$ of $\mathcal{H}^{A,A'}$ are also Verifier's strategies in $\MilestoneG^{\strat{\Refuter},\strat{\Verifier}}_{A,A'}$,
%hence: 
%\[\adjustlimits
%\inf_{\strat{\Verifier} }\sup_{\strat{\Refuter}} \mathbb{E}_{\mathcal{H}^{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] \leq \adjustlimits \inf_{\strat{\Verifier}} \sup_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask].
%\] 
%On the other hand, as shown above, for any Verifier's strategy $\pi$ in $\MilestoneG^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}$ we have: 
%\[
% \inf_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] \leq \inf_{\strat{\Refuter}} \mathbb{E}_{\mathcal{H}_{A,A'}}^{\stratprime{\Verifier},\strat{\Refuter}}[\FMask]
%\]
%and then:
%\[ \adjustlimits
% \sup_{\strat{\Verifier}} \inf_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] \leq \adjustlimits \sup_{\strat{\Verifier}} \inf_{\strat{\Refuter}} \mathbb{E}_{\mathcal{H}_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]
%\] 
% And therefore:
%\[ \adjustlimits
%   \inf_{\strat{\Refuter}} \sup_{\strat{\Verifier}} \mathbb{E}_{\mathcal{H}^{A,A'}}^{\strat{\Refuter},\strat{\Verifier}}[\FMask] 
%   \leq  \adjustlimits
%   \inf_{\strat{\Refuter}} \sup_{\strat{\Verifier}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask] \leq \adjustlimits  \sup_{\strat{\Verifier}} 
%   \inf_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]
%    \leq \adjustlimits \sup_{\strat{\Verifier}} \inf_{\strat{\Refuter}} \mathbb{E}_{\mathcal{H}_{A,A'}}^{\strat{\Verifier},\strat{\Refuter}}[\FMask]
%\]
%Since $\mathcal{H}^{A,A'}$ is determined, we get:
%\[ \adjustlimits
% \inf_{\strat{\Verifier}} \sup_{\strat{\Refuter}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Refuter},\strat{\Verifier}}[\FMask] = \adjustlimits   \sup_{\strat{\Refuter}} \inf_{\strat{\Verifier}} \mathbb{E}_{\MilestoneG_{A,A'}}^{\strat{\Refuter},\strat{\Verifier}}[\FMask]
%\]
%That is, $\MilestoneG^{\strat{\Verifier},\strat{\Refuter}}_{A,A'}$ is determined and the value of this game coincides with the value of $\mathcal{H}_{A,A'}$.
%\end{proof}

	Interestingly, we can  use the symbolic graph to decide  whether a probabilistic masking game (which could be infinite) is almost-surely failing or not. To do so,
given any symbolic graph $\SymbG_{A,A'}$ as in Def.~\ref{def:symbolic_game_graph}, we define $\pre_\Box(V')$, for $V' \subseteq V^{\SymbG_{A,A'}}$ and $\post_\Diamond(v)$ for $v \in V^{\SymbG_{A,A'}}$,
as follows:
\begin{align*}
	\pre_\Box(V') =&  (\pre(V') \cap (V^{\SymbG_{A,A'}}_\Verifier \cup V^{\SymbG_{A,A'}}_\Refuter)) \\
				&\cup (\pre(V') \cap \{ v \in V_P^{\SymbG_{A,A'}} \mid \Eq(v)(V') \text{ has no solutions}\})
\end{align*}
and:
\begin{align*}
	\post_\Diamond(v) =&  (\post(v) \cap (V^{\SymbG_{A,A'}}_\Probabilistic \cup V^{\SymbG_{A,A'}}_\Verifier)) \\
				&\cup \{ v' \in \post(v) \cap V^{\SymbG_{A,A'}}_\Refuter \mid \LP(v)(v') \text{ has solutions}\})
\end{align*}
where $ \LP(v)(v')$ is the linear programming problem consisting of the equations $\Eq(v)$ plus the inequality $x_{\pr{0}{v'},\pr{2}{v'}}>0$. Intuitively,
$\pre_\Box(V')$  characterizes those predecessors of $V'$ for which the probability of reaching the vertices of $V'$ is greater than $0$ in any Markov chain obtained by selecting
some strategies. On the other hand, $\post_\Diamond(v)$ describes those vertices that are successors of $v$ in some Markov chain obtained from a pair of strategies.
Furthermore, let $\pre_\Box^*$ and $\post_\Diamond^*$ denote the transitive closures of these operators. 

\begin{theorem} \label{thm:prob_reach_error_gm}  
Let $A = \langle S, \Sigma, \rightarrow, s_0 \rangle$ and $A' = \langle S', \Sigma, \rightarrow', s'_0 \rangle$ be two PTSs, and 
$\MilestoneG_{A,A'}= (V^\StochG, E^\StochG, V^\StochG_\Refuter, V^\StochG_\Verifier, V^\StochG_\Probabilistic, \InitVertex, \delta^\StochG, r^\StochG, \mathcal{M})$ a game with milestones, and $\SymbG_{A,A'}$ be the corresponding symbolic game graph. 
Then,  the probability of reaching the error state in 
 $\MilestoneG_{A,A'}^{\strat{\Verifier},\strat{\Refuter}}$ is $1$, for all strategies  $\strat{\Verifier},\strat{\Refuter},$ iff $\post^*_\Diamond(v^{\SymbG_{A,A'}}_0) \subseteq \pre^*_\Box(\{\ErrorSt\})$.
 %for all probabilistic states $v \in \post^*(v^{\SymbG}_0)$ the equations 
% $\Eq(v, V^\SymbG \setminus( \pre^*(V^\SymbG \setminus \pre^*(\ErrorSt))))$ has no solutions.
\end{theorem}	
%\begin{proof}
%For proving this theorem we follow the notation introduced in \cite{Katoen}, let $\Prob{\strat{\Verifier}}{\strat{\Refuter}}(v \vDash \Diamond \ErrorSt)$ denote the probability of
%reaching $\ErrorSt$ in $\MilestoneG_{A,A'}^{\sigma,\pi}$ from vertex $v$. We also define for every symbolic vertex the set
%$[v] = \{ v' \in V^\StochG \mid \forall 0 \leq i \leq 4 \pr{i}{v} = \pr{i}{v'} \}$.
%\\
%\noindent (Only If) Assume that $\MilestoneG_{A,A'}$ is  almost-sure failing, for the sake of contradiction suppose that 
%$\post^*_\Diamond(v^{\SymbG_{A,A'}}_0) \cap (V^{\SymbG_{A,A'}} \setminus \pre^*_\Box(\ErrorSt)) \neq \emptyset$, and let
%$v \in \post^*_\Diamond(v^{\SymbG_{A,A'}}_0) \cap (V^{\SymbG_{A,A'}} \setminus \pre^*_\Box(\ErrorSt))$, since
%$v \in  \post^*_\Diamond(v^{\SymbG_{A,A'}}_0)$
% we have strategies $\strat{\Verifier}$ and $\strat{\Refuter}$ such that (for 
%$\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$ we have $v' \in\post^*(v_0)$, being $v_0$ the initial state of the Markov chain,
%but since $v \in (V^{\SymbG_{A,A'}} \setminus \pre^*_\Box(\ErrorSt))$, and by definition of $ \pre^*_\Box$, we have that 
%in $\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$ $v' \in (V^{\MilestoneG} \setminus \pre^*(\ErrorSt))$, thus
%$\post^*(v_0) \cap (V \setminus \pre^*(\ErrorSt)) \neq \emptyset$ (being $V$ the set of states of Markov chain $\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$), this contradicts
%Theorem~10.29 in \cite{Katoen}.
%
%\noindent (If) Suppose that  $\strat{\Verifier},\strat{\Refuter},$ iff $\post^*_\Diamond(v^{\SymbG_{A,A'}}_0) \subseteq \pre^*_\Box(\{\ErrorSt\})$, and let $\strat{\Verifier}, \strat{\Refuter}$
%a pair of strategies, and consider the Markov chain $\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$. Now, consider $v \in \post^*(v_0)$ in this Markov chain,
%by definition of  $\SymbG_{A,A'}$, there is a $v' \in V^{\SymbG_{A,A'}}$ such that $v \in [v']$, since  $v \in \post^*(v_0)$ we have a path $v_0,v_1,\dots, v$ in 
%$\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$, and therefore we have a path $v^{\SymbG_{A,A'}}_0, v'_1,\dots, v'$ in $\SymbG_{A,A'}$ with $v_i \in [v'_i]$,
%hence $v' \in \post^*_\Diamond(v^{\SymbG_{A,A'}}_0)$ (note that the existence of the path $v_0,v_1,\dots, v$ in the Markov chain implies this), thus
%by assumption we have that $v' \in \pre^*_\Box(\ErrorSt)$ this implies that $v \in \pre^*(\ErrorSt)$ in $\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$ and thus
%$\post^*(v_0) \subseteq \pre^*(\ErrorSt)$ in $\MilestoneG^{\strat{\Verifier}, \strat{\Refuter}}_{A,A'}$, using Theorem~10.29 in \cite{Katoen}, 
%we obtain that the probability of reaching the error state in $\MilestoneG_{A,A'}^{\strat{\Verifier},\strat{\Refuter}}$ is $1$.
%\end{proof}

%\todo[inline]{$\pi$ is used both for projection and player 2's strategies}

Furthermore, the expected value of $\FMask$ can be computed via a set of functional equations.
\begin{theorem}  \label{thm:solution_eq_stock_game} Let $\MilestoneG_{A,A'}$ a stochastic masking game with milestones for some PTSs $A$ and $A'$, and let $\SymbG_{A,A'}$ be 
the corresponding symbolic game. Then, $\sup_{\strat{\Verifier}} \inf_{\strat{\Refuter}}\Expect{\strat{\Verifier}}{\strat{\Refuter}}[\FMask]$ is the solution of a set of functional equations, defined as follows:
\[
    x(v) =
    \begin{cases}
           %\displaystyle \max_{w \in \vertices{\couplings{\pr{3}{v},\pr{4}{v}}}} \{\chi_{\mathcal{M}}(\pr{1}{v}) + \sum_{v' \in \post(v)} w(v,v')  x_{v'} \}& \text{ if }v \in V^{\SymbG}_\Verifier  \\
           %\displaystyle \max_{w \in \vertices{\couplings{\pr{3}{v}}{\pr{4}{v}}}} \{\chi_{\mathcal{M}}(\pr{1}{v}) + \sum_{v' \in \post(v)} w(\pr{0}{v'},\pr{2}{v'})  x_{v'} \}& \text{ if }v \in V^{\SymbG}_\Verifier  \\
           \displaystyle \max_{w \in \vertices{\couplings{\pr{3}{v}}{\pr{4}{v}}}} \{\sum_{v' \in \post(v)} w(\pr{0}{v'},\pr{2}{v'})  x(v') \}& \text{ if }v \in V^{\SymbG}_\Probabilistic  \\
           \displaystyle \max \{\chi_{\mathcal{M}}(\pr{1}{v})  + x(v') \mid v' \in \post(v) \} & \text{ if } v \in  V^{\SymbG}_\Verifier, \\
           \displaystyle \min \{\chi_{\mathcal{M}}(\pr{1}{v})  + x(v') \mid v' \in \post(v) \} & \text{ if } v \in  V^{\SymbG}_\Refuter, \\
           \displaystyle 0 & \text{ if } v=\ErrorSt.
           \displaystyle 
    \end{cases}
\]
\end{theorem}
%\begin{proof} The proof of this theorem follows the same ideas as the proof of theorem \ref{theo:determined}. We can define the game $\mathcal{H}_{A,A'}$ restricting Probabilistic vertices of $\MilestoneG_{A,A'}$ to 
%the vertices of the $2$-way transportation polytopes. As proven in Theorem \ref{theo:determined}, this is a transient game, and also its value coincides with the value of $\MilestoneG_{A,A'}$. Furthermore when
%considering  $\mathcal{H}_{A,A'}$ as a transient game defined as follows: the games is played by two players the maximizer (associated to the Verifier), and 
%the minimizer (associated to the Refuter),   the states of the transient game are the states of the symbolic game, say $v_0,\dots,v_n$, where the actions
%associated to each state are defined as follows: if $v$ is a Verifier's vertex, then the maximizer has one action per successor, and the minimizer has no actions;
%for Refuter's vertices the the minimizer has one action per successor, and the maximizer has no actions; for Probabilistic nodes the maximizer has one action per 
%successor and the Verifier has no actions. The payoff is $\FMask$, as proven in Theorem \ref{theo:determined}, this game is transient (as defined in \cite{CompetitiveMarkovBook}), and therefore
%has a value and it can be computed by the functional equations given above, this finish the proof. 
%\end{proof}

	These functional equations can be solved using a value iteration algorithm \cite{Condon90}, this method computes the  least fixed point of a function $U: \mathbb{R}^n \rightarrow \mathbb{R}^n$ defined via these equations; $U$ is a contraction map, and therefore it has a unique fixed point \cite{FilarV96}.
	
%	Function $\FMask$ is Borel measurable.
%\begin{theorem}	$\FMask$ is Borel measurable.
%
%\end{theorem}	
%Using Martin's Theorem we can show that:
%\begin{theorem}
% Any stochastic masking game with reward function  $r^G$ and \emph{masking payoff function} as defined above is
%determined, that is:
%\[
%	\text{sup}_{\sigma \in \Sigma} \text{inf}_{\pi \in \Pi}  \mathbb{E}^{\pi, \sigma}[\FMask]  =  \text{inf}_{\pi \in \Pi} \text{sup}_{\sigma \in \Sigma} \mathbb{E}^{\pi, \sigma}[\FMask]
%\]
%\end{theorem}

	

%	Interestingly, the symbolic game introduced in Section \ref{} can be modified to compute the optimal strategies for Player 1 and Player 2. 
%First, let us describe the algorithm that we use to compute the optimal strategies. Then, we consider functions $U^j_i:\mathcal{I} \rightarrow S^{\mathcal{G}} \rightarrow [0,1]$ with $i,j \in \mathbb{N}$, which can be thought of as a quantitative generalization  of the sets $U^i_j$ defined in Section \ref{}.
%
%\begin{definition} Given stochastic masking game $\mathcal{G}_{A,A'}
%  = \langle S^{\mathcal{G}}, S^{\mathcal{G}}_R, S^{\mathcal{G}}_V, \Sigma^\mathcal{G}, E^{\mathcal{G}}, {s_0}^{\mathcal{G}}, v^G,  r^G \rangle$. We define functions $U^j_i : S^G \rightarrow [0,1]$ as follows:
%  \begin{equation*}
%      \text{U}^0_0(s) = \begin{cases*}
%                        1       & \text{if $s=s_{err}$}\\
%                        0       & \text{otherwise}
%                      \end{cases*}
%    \end{equation*}
%    \begin{equation*}
%    	 \text{U}^0_{i+1}(s) = 0 \; \; \forall s \in S^{\mathcal{G}}
%    \end{equation*}
%    \begin{equation*}
%      \text{U}^{j+1}_{i}(s) = \begin{cases*}          
%                        {\displaystyle  \sum_{s' \in post(s)} \pi_{5}(s)(\pi_{0}(s'), \pi_{2}(s')  ) \cdot \text{Max}\{U^j_{k}(s') \mid k\leq i \}}   & \text{if $s \in S_{P}$} \\
%                        {\text{Min}\; \{ U^j_{i}(s') \mid s \rightarrow s' \}}  & \text{if $s \in S_{V} \wedge \pi_{1}(s) \notin \mathcal{F}$} \\                
%                        {\text{Min}\;  \{ \frac{1}{2} \cdot U_{i-1}(s') \mid  s \rightarrow s'  \}}  & \text{if $s \in S_{V} \wedge \pi_{1}(s) \in \mathcal{F} \wedge i>0$}  \\
%                        {0}  & \text{if $s \in S_{V} \wedge \pi_{1}(s) \in \mathcal{F} \wedge i=0$}  \\
%                        {\text{Max}\; \{ U^j_{i}(s') \mid s \rightarrow s'  \}}          	    & \text{if $s \in S_{R}$}  \\
%                      \end{cases*}
%  \end{equation*}
%  where:
%  \begin{equation*}
%  	U_i(s) = \text{Max}\; \{ U^j_i(s) \mid j \geq 0\}
%  \end{equation*}
%  and
%   \begin{equation*}
%  	U(s) = \text{Max}\; \{ U_i(s) \mid i \geq 0\}
%  \end{equation*}
%\end{definition} 
%
%\begin{theorem} For any  stochastic masking game with rewards $\mathcal{G}_{A,A'}$ and payoff function $\FMask$, Player 1 and Player 2
%have optimal memoryless pure strategies
%\end{theorem}

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/loopExample.pdf}
%\caption{Example of PTS's with loops} \label{fig:exam_2_loop}
%\end{figure}
%
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/loopExampleGameGraph.pdf}
%\caption{Partial Game Graph for PTS's of Fig. ~\ref{fig:exam_2_loop}} \label{fig:exam_2_loop_gamei}
%\end{figure}

%	
%\begin{definition} \label{def:strong_masking_game_graph}
%  Let $A = \langle S, \Sigma, \rightarrow, s_0 \rangle$ , $A' = \langle S', \Sigma, \rightarrow', s'_0 \rangle$ be two PTSs.
%  The \emph{symbolic bisimulation game graph} $\mathcal{G}_{A,A'}
%  = \langle S^G, S_R, S_V, \Sigma^G, E^G, {s_0}^G \rangle$ for two
%  players is defined as follows:
%
%\begin{itemize}
%    \item $\Sigma^G = \Sigma$
%  \item $S^G = (S \times ( \Sigma^1 \cup \Sigma^2 \cup\{\#\}) \times S' \times \Dist(S) \times \Dist(S') \times \Dist(S \times S') \times \{ R, V \}) 
%  \cup \{\ErrorSt\}$
%  \item $s_0^G = \langle s_0, \#, s'_0, \mhyphen, \mhyphen, \mhyphen, R \rangle$, 
%  \item $S_R = \{ (s, \#, s', \mu, \mu', w, R) \mid s \in S \wedge s' \in S' \wedge \mu \in \Dist(S) \wedge \mu' \in \Dist(S') \wedge w \in \Dist(S \times S') \} 
%  \cup \{\ErrorSt\}$,
%  \item $S_V = \{ (s, \sigma, s', \mu, \mhyphen, \mhyphen, V) \mid s \in S \wedge s' \in S' \wedge \sigma \in \Sigma^G \wedge \mu \in \Dist(S)\} \cup \{ (s, \sigma, s', \mhyphen, \mu', \mhyphen, V) \mid s \in S \wedge s' \in S' \wedge \sigma \in \Sigma^G \wedge \mu' \in \Dist(S')\}$
%\end{itemize}
%and $E^G$ is the minimal set satisfying:
%\begin{itemize}
%  \item $\{ (s, \#, s', \mhyphen, \mhyphen, \mhyphen, R) \xrightarrow{\sigma,\nu} (s, \sigma^{1}, s', \mu, \mhyphen, \mhyphen, V) \mid \exists\;\sigma \in \Sigma: s \xrightarrow{\sigma} \mu \in \rightarrow\} \subseteq E^G$,
%
%  \item $\{ (s, \#, s', \mhyphen, \mhyphen, \mhyphen, R) \xrightarrow{\sigma,\nu} (s, \sigma^{2}, s', \mhyphen, \mu', \mhyphen, V) \mid \exists\;\sigma \in \Sigma: s' \xrightarrow{\sigma} \mu' \in \rightarrow'\} \subseteq E^G$,
%  
%  \item $\{ (s, \#, s', \mu, \mu', w, R) \xrightarrow{t,t',\sigma,\nu} (t, \sigma^{1}, t', \nu, \mhyphen, \mhyphen, V) \mid (\exists\;\sigma \in \Sigma: t \xrightarrow{\sigma} \nu \in \rightarrow) \wedge (w(t,t') > 0)\} \subseteq E^G$,
%
%  \item $\{ (s, \#, s', \mu, \mu', w, R) \xrightarrow{t,t',\sigma,\nu'} (t, \sigma^{2}, t', \mhyphen, \nu', \mhyphen, V) \mid (\exists\;\sigma \in \Sigma: t' \xrightarrow{\sigma} \nu' \in \rightarrow') \wedge (w(t,t') > 0) \} \subseteq E^G$,
%
%  \item $\{ (s, \sigma^2, s', \mhyphen, \mu', \mhyphen, V) \xrightarrow{\sigma,\mu,w} (s, \#, s', \mu, \mu', w, R) \mid (\exists\;\sigma \in \Sigma: s' \xrightarrow{\sigma} \mu \in \rightarrow) \wedge (w \in \Dist(S \times S') \wedge w$ is coupling for $(\mu,\mu'))\} \subseteq E^G$,
%
%  \item $\{ (s, \sigma^1, s', \mu, \mhyphen, \mhyphen, V) \xrightarrow{\sigma,\mu',w} (s, \#, s', \mu, \mu', w, R) \mid (\exists\;\sigma \in \Sigma: s' \xrightarrow{\sigma} \mu' \in \rightarrow') \wedge (w \in \Dist(S \times S') \wedge w$ is coupling for $(\mu,\mu'))\} \subseteq E^G$,
%
%    \item If there is no outgoing transition from some state $s$ then transitions $s \xrightarrow{\sigma} \ErrorSt$ and $\ErrorSt \xrightarrow{\sigma} \ErrorSt$ for every $\sigma \in \Sigma$, are added.
%\end{itemize}
%
%\end{definition}	


%	Let us consider the games in Figure \ref{fig:two-models}, part of the game for these structures is shown in Figure \ref{fig:game}.
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/two-models.pdf}
%\caption{Two non-bisimilar models} \label{fig:two-models}
%\end{figure}
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/game.pdf}
%\caption{Game for the example} \label{fig:game}
%\end{figure}
%	Note that this graph is infinite, because the number of couplings the Verifier can choose is clearly infinite. However, we show that 
%the game can be represented and solved by means of a finite game graph, as is show below.
%\subsection{A Symbolic Game Graph}
%	The symbolic masking game is similar to the game defined above, but instead of considering each possible coupling, we use a system of equations whose solutions correspond to 
%the possible couplings. First, let us define for each pair of transitions $\mu \in \mbox{Dist}(S)$ and $\mu' \in \mbox{Dist}(S')$ a system of equations $\text{Eq}(\mu,\mu')$ as follows.
%\begin{definition} Given sets $S$ and $S'$,  distributions $\mu \in \text{Dist}(S)$, $\mu' \in \text{Dist}(S')$ and variables $X=\{x_{i,s}\}$. $\text{Eq}(\mu, \mu')$ is the following $(n+m)$-vector of equations: 
%	\begin{equation*}
%		\text{Eq}(\mu,\mu')_{k} = \begin{cases*}
%      							  {\displaystyle (\sum^{m-1}_{j=0} x_{k,j})=\mu(s_k)} 		      & if k$<$n \\
%     							  {\displaystyle (\sum^{n-1}_{i=0} x_{i,k-n})=\mu'(s_{k-n}) }	      & otherwise
%   						      \end{cases*}
%	\end{equation*}
%where 
%\end{definition} 
%When useful can write these equations in matrix form: 
%\[
%\text{Eq}(\mu,\mu') = (\mathbf{A}_{\mu,\mu'} \mathbf{X}_{\mu,\mu'} = \mathbf{C}_{\mu,\mu'}). 
%\]
%Furthermore, given
%a set of variables $X' \subset X_{\mu,\mu'}$, we define the equation $\sum_{x \in X'} x = 0$, and call $\widehat{\text{Eq}}(\mu,\mu')$ to the system of equations
% $\text{Eq}(\mu,\mu')$ extended with $\sum_{x \in X'} x = 0$.
%
%	The, the symbolic graph game is defined as follows.
%%\begin{definition} \label{def:masking_game}
%%The game consists in the repetition of the following steps:
%	\begin{itemize}
%		\item Step 1: $R$ chooses an action $a$ and  a distribution $\mu$ such that $s \xrightarrow{a} \mu$ (resp. $s' \xrightarrow{a} \mu$).
%		\item Step 2: $V$ chooses a matching action $a$ (or $M$ if $a \in F$), distribution $\mu'$ .
%		\item Step 3: $R$ chooses $(t, t')$ such that there is some  $w(t, t') > 0$, from which the next sequence, f steps will begin.
%	\end{itemize}
%%\end{definition}
%Notice that steps 3, and 1 can be collapsed into a single step. The Verifier wins if the play is infinite, otherwise the Refuter wins. 	
%	For solving the game we add an error state ($s_{\mbox{err}}$) and compute the following sets.
%\begin{align*}
%	U^0 & = \{s_{err}\}\\
% 	U^{1} & = \{v \mid v \mbox{ is  a verifier's state that cannot match the refuter's play}   \} \\
%	U^{i+1} &= \{ v \mid v \mbox{ is  a refuter's state such that $Eq(s,t,\mu,\mu')$ has a solution} \}\\
%		    & \;\; \;\; \cup \{ v \mid s \mbox{ is  a verifier's state such that all its successors go to $U^i$}\} \\
%\end{align*}
%	Where $Eq(v)$ are defined as follows. $v$ is a Refuter's state, and then it has distributions $\mu$ and $\mu'$,
%where  $|\mu| = \{c_0, \dots, c_n\}$ and $|\mu| = \{c'_0,\dots,c'_m\}$.	
%	 Then, let a $\mathbf{X}$ be a
%$2 \times (n*m)$ matrix, defined as follows:
%\[
%	\mathbf{X}_{i,j} 
%\]
%
%	Let us consider the games in Figure \ref{}, then part of the game for these structures is shown in Figure \ref{}.
%




